Quantized Sparse Weight Decomposition for Neural Network Compression

In this paper, we introduce a novel method of neural network weight compression. In our method, we store weight tensors as sparse, quantized matrix factors, whose product is computed on the fly during inference to generate the target model's weights. We use projected gradient descent methods to find quantized and sparse factorization of the weight tensors. We show that this approach can be seen as a unification of weight SVD, vector quantization, and sparse PCA. Combined with end-to-end fine-tuning our method exceeds or is on par with previous state-of-the-art methods in terms of the trade-off between accuracy and model size. Our method is applicable to both moderate compression regimes, unlike vector quantization, and extreme compression regimes.

==> Vector quantization_/conclusion.tex <==
\vspace{-0.35cm}
%\FloatBarrier

\section{Conclusion}
\vspace{-0.2cm}
We presented a weight compression method based on quantized sparse PCA which unifies SVD-based weight compression, sparse PCA, and vector quantization.
We tested our method on ImageNet classification and show  compression-accuracy  trade-offs which are state-of-the-art or on par with strong baselines,  and demonstrated that our method is the only method to achieve SOTA compression-accuracy trade-offs in both low and high compression regimes.
Lastly, we investigated whether low rank approximations, quantization, or sparsity yield the best efficiency-accuracy trade-offs, and found that at high compression ratios, increasing rank and decreasing bit-width can improve results.
For future work, we plan to investigate methods for automated rank, bit-width, and sparsity ratio selection in order to further improve the accuracy and reduce the hyper-parameter search time.


==> Vector quantization_/experiments.tex <==
%\vspace{-0.25cm}
\begin{figure*}[t]
\centering
\begin{small}
\begin{tabular}{l}
\hspace{-0.2cm}\includegraphics[width=0.75\textwidth]{fig/mobilenet_v2_iclr.pdf}
\end{tabular}
\end{small}
\caption{Results for MobileNetV2 trained on ImageNet.}
\label{fig:mobilenet_v2_results}
\end{figure*}
\section{Experiments}\label{sec:experiments}
\vspace{-0.25cm}
In this section we describe two sets of experiments: one set to explore the effect of compression hyperparameters on compression-accuracy trade-offs, and one set of experiments to compare against various baseline methods.
\subsection{Experimental setup}
\vspace{-0.15cm}
%In all our experiments we start from a pre-trained model. 
%The experimental details for each step in Section~\ref{sec:methodoutline} is described below.
%\vspace{-0.2cm}
\paragraph{Initial factorization}
We start with a pre-trained model and perform the factorization as described in Section \ref{sec:qs_pca_solver}.
We initialize the per-channel quantization scale using min-max quantization~\citep{krishnamoorthi2018quantizing}.
\vspace{-0.2cm}
\paragraph{Per layer data-aware optimization}
To perform the data-aware optimization, we sample a single batch of 64 input and output activations for a layer. We split the data into a training set and a validation set (we keep one eighth of the data as the validation set).  
We keep track of the error on the validation set.
During this step we use the Adam optimizer~(\cite{kingma2014adam}) with learning rate $10^{-4}$ and weight decay $10^{-5}$.
\vspace{-0.2cm}
%\FloatBarrier
\paragraph{Sparsification} Sparsification is applied after per layer data-aware optimization in a form of hard thresholding. We consider one-shot and iterative thresholding. Specifically, for each layer, the quantized weights are sorted by absolute value, then a desired percentage of values is masked out. We do not prune weights that become zeros after the quantization step, instead, we add extra sparsity on top of accidental sparsity that occurs after the quantization. During the consequent fine-tuning stage, the sparsity mask is frozen.
%\vspace{-0.2cm}
\paragraph{Fine-tuning}
We follow \cite{martinez2021permute} and fine-tune our models end-to-end using the target training set.
Model-specific finetuning procedures are described below.



%We use the same hyperparameter settings for ResNet50.
% add about dimensionality we search for
% add range of K we search for
% add weight decay, LR schedule etc
% add table of full results to appendix
%\vspace{-0.25cm}
\subsubsection{A note on compression ratio}
%\vspace{-0.15cm}
In our experiments we leave the first convolutional weight tensor, all bias tensors, all batch normalization parameters, and the PCA centering vectors in FP32. 
We denote these uncompressible parameters as $L_u$.
The sparsity ratio for a network is then computed as $C_r=\frac{\sum_{\mathbf{W}} L_o(\mathbf{W})}{L_u + \sum_{\mathbf{W}}L_c(\mathbf{W})}$
%\vspace{-0.25cm}
\subsection{ImageNet Experiments}
%\vspace{-0.15cm}
We evaluate our method on the ResNet18 and MobileNetV2 achitectures for ImageNet classification. 
We apply our method on pretrained versions of the model, where we take the pretrained weights from the PyTorch model zoo.
In all our experiments we keep the tile size $d$ constant at 256, the bitwidth of the codebook matrix $\textbf{C}$ constant at 4, and use per-channel scalar quantization of 4 bits for the fully connected classification layer weights.
To achieve different compression ratios we vary the rank $k$ with values between 64-256, the bitwidth of the latent matrix $\textbf{Z}$ between 3-6, and the extra sparsity of $\textbf{Z}$ between 0\% and 40\%. 
Further experimental details can be found in Section~\ref{sec:expdetailsappendix}.


%\vspace{-0.15cm}
\subsubsection{Baseline methods}
%\vspace{-0.15cm}
We compare our methods against scalar quantization by~\cite{esser2019learned},  binary CNNs by~\cite{lin2017towards} (ABC-Net), the vector quantization method by~\cite{martinez2021permute} (PQF), the vector quantization method by~\cite{stock2019and} (BGD), trained ternary quantization by~\cite{zhu2016trained} (TTQ).
The results for scalar quantization are produced using LSQ \cite{esser2019learned}, with 4, 3 and 2-bit per-channel weight quantization and FP32 bit activations. For these experiments a weight decay of $10^{-4}$ and cosine learning rate decay to $10^{-2}$ of the original learning rate was used.
\vspace{-0.15cm}

\subsubsection{Results}
\vspace{-0.15cm}
The Pareto dominating results of our method and comparison to the baselines can be found in Figure~\ref{fig:resnets_plots} and Figure~\ref{fig:mobilenet_v2_results}. 
The full set of (non Pareto dominating) results for Resnet18 can be found in Figure~\ref{fig:ablationa}.
The same results along with the values for rank, bitwidth and sparsity and resulting compression ratios can be found in Table~\ref{tab:all_results_rn18} in the Appendix.
In this figure we see that we outperform BGD, TTQ, ABC-Net and 3 and 2 bit scalar quantization by considerable margins.
Furthermore, we outperform or match the strongest baseline at high compression ratios, PQF for compression ratios of 17x and higher, and are on par with 4-bit scalar quantization for compression ratios under 17x. 
Lastly, we are the only method to achieve SOTA compression-accuracy trade-offs over the full range from 5x to 40x compression.
\vspace{-0.35cm}
\subsection{Ablation studies}
\vspace{-0.15cm}
\subsubsection{Hard thresholding methods}
\vspace{-0.15cm}
\begin{table*}%[!htbp]
  \centering
  \begin{tabular}{cccccccc}
    \toprule
    & &  \multicolumn{3}{c}{\parbox{2.8cm}{\centering Pre-FT accuracy}} & \multicolumn{3}{c}{\parbox{2.8cm}{\centering Post-FT accuracy}}
    \\
    \parbox{1.7cm}{\centering Hard thresholding\\method} & \parbox{1.5cm}{\centering Stopping.\\critetion} & \parbox{1.1cm}{\centering 10\%\\sparsity} & \parbox{1.1cm}{\centering 20\%\\sparsity} & \parbox{1.1cm}{\centering 30\%\\sparsity} & \parbox{1.1cm}{\centering 10\%\\sparsity} & \parbox{1.1cm}{\centering 20\%\\sparsity} & \parbox{1.1cm}{\centering 30\%\\sparsity} \\ 
    \midrule
    One-shot HT & val. set &  63.2 & 58.9 & 47.3 & \textbf{69.1} & 68.7 & \textbf{68.1}\\ 
    One-shot HT & 100 iter. & 59.4 & 55.5 & 45.2 & 68.8 & 68.4 & 68.0\\ 
    Iterative HT & 30 iter. & \textbf{64.5} & \textbf{63.0} & \textbf{58.8} & \textbf{69.1} & \textbf{68.8} & 68.0 \\ 
    Iterative HT &  100 iter. & 62.0 & 60.7 & 57.3 & 69.0 & 68.7 & \textbf{68.1}\\ 
    Iterative HT &  1000 iter. & 55.0 & 55.4 & 54.1 & 68.5 & 68.3 & 67.9\\ 
    No data-aware opt. & - & 58.5 & 53.3 & 37.8 & 69.0 & 68.7 & 67.9\\ \bottomrule
\end{tabular}
\caption{Resnet18 ablation on the impact of the hard thresholding method and the stopping criterion on top-1 validation accuracy of the compressed model. Iterative hard-thresholding with 30 iterations shows the best results among all the other methods, however, the benefit vanishes after fine-tuning.}
\label{tab:ht_ablation}
\end{table*}
%\vspace{-0.15cm}

% \textbf{Per layer results}

% In this section we compare different compression methods on the single largest layer of Resnet18 in terms of the trade-off between the compression ratio and mean-squared error of the output activations. We use the same amount of data as we use for per layer data optimization.
 
% \begin{figure}
% \centering
% \begin{small}
% \includegraphics[width=7.5cm]{fig/per_layer_plots.pdf}
% \end{small}
% \caption{Per layer results for Resnet18}
% \label{fig:per_layer_plots}
% \end{figure}

% \vspace{-1.5cm}

% \subsection{Image classification}
% The final results of the exploration are shown in figure \ref{fig:resnet_plots}.

In this section, we study the impact of the hard thresholding method and the stopping criterion for data-aware optimization. Algorithm \ref{alg:projected_gd} applies the hard-thresholding step at each iteration. However, we can also apply it only after the end of gradient descent iterations. We call this one-shot hard-thresholding. The method has precedence in non-convex sparse optimization  (\cite{shen2020one}). We consider two different stopping criteria. The first is using the fixed number of gradient descent iterations, e.g., 30, 100, or 1000. The second is based on achieving the MSE error threshold on the validation set. We split the data used for per-layer optimization into a training set and a validation set. We stop the iterations as soon as the error on the validation set is not decreasing for more than two iterations. Finally, we compare both methods with one-shot hard-thresholding without data-aware optimization. 

We present the results for Resnet18 in the Table~\ref{tab:ht_ablation}. Three different levels of sparsity are considered for a model with 4 bit latent. We report the validation accuracy of the model before and after fine-tuning. 
The results suggest that the most important aspect of data-aware optimization is the stopping criterion. The best pre-finetuning results are obtained by using iterative hard thresholding with the least number of iterations, namely 30. The second best method is one-shot iterative hard thresholding with the stopping criterion based on the validation set. These results suggest that it is important to limit the number of iterations of per layer optimization in order to prevent the method from over-fitting to the layer input and output data sample. This intuition is further supported by observing the lowest pre-finetuning accuracy for hard thresholding with the highest number of iterations, namely 1000.

However, overall benefits of per layer optimization methods become marginal after the compressed model is fine-tuned. In various experiments, we observed an  0.1-0.3\% improvement in the validation accuracy compared to using one-shot hard thresholding without any data-aware optimization.
Therefore, in our further full model experiments, we used one-shot hard thresholding with the stopping criterion based on the validation set as a method of low computational complexity, which gives nearly the best results compared to the other methods.

\vspace{-0.25cm}
\subsubsection{Quantization vs Pruning vs Rank}
%\vspace{-0.25cm}
In our method, compression can be achieved by lowering rank, lowering the bit-width for latent matrices (hence referred to as `bit-width'), or increasing extra sparsity. 
Thus, similar compression ratios can be achieved with different values for rank, bit-width and sparsity.
For example, for a given model, we can retain the same compression ratio by increasing rank and decreasing bit-width to compensate.
In this section we investigate whether we can discover patterns that would help guide compression hyperparameter search.

In Figure~\ref{fig:ablationa} we show a scatter plot with the full set of results.
% In this plot we show the results for the best learning rate and learning rate schedule for each compression hyperparameter setting.
In this figure, we see that for  low compression ratios (below 14x) only minor improvements can be achieved by tweaking compression hyperparameters. 
For example, around 10x compression even the worst performing compression hyperparameters are still on par with quantization to 3 bits (10.67x compression). 
However, for higher compression ratios the compression hyperparameters have a larger impact on model performance.

In Figure~\ref{fig:ablationb} we show the effect of rank, bit-width and sparsity ratios on a set of models with a low (near 11x, top row) and a high (near 25x, bottom row) compression ratio.
Again we see little effect (roughtly 0.5\%) for the lower compression ratio.
However, for the more aggressively compressed models in the bottom row, we see that increasing rank while lowering bit-width to compensate has a strong positive effect on model performance.
Finally, in both plots we see no clearly discernible trend in the effect of compression ratio on model accuracy.

Based on these results we conclude that, at high compression ratios, increasing rank and decreasing bit-widths can improve results.
Sparsity can be used to further fine-tune the target compression ratio.

\begin{figure}
  \begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\linewidth]{fig/resnet18_plots_all.pdf}
  \end{subfigure}%
  %\hspace*{\fill}   % maximize separation between the subfigures
   \caption{All results for ResNet18, including non-Pareto dominating results.}\label{fig:ablationa}
\end{figure}

\begin{figure}
    \begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\linewidth]{fig/resnet18_ablation_11x-25x.pdf}
    
  \end{subfigure}%
  \caption{Resnet18, the effect of rank, bit-width and sparsity for models near 11x (top row) and 25x (bottom row) compression ratios.}\label{fig:ablationb}
  %\caption{Full results and effect of rank, bit-width and sparsity.}
\end{figure}

% \begin{table}[]
%     \centering
%     \begin{tabular}{rrrrrr}
%         \toprule
%          \multicolumn{6}{c}{compression ratios near 25x} \\
%           K &    D &  bw &  sparsity &  comp. rate &  accuracy \\
%         \midrule
%          39 &  256 &   6 &      0.00 &  25.97 &      54.04 \\
%          40 &  256 &   6 &      0.10 &  25.52 &      54.06 \\
%          48 &  256 &   5 &      0.00 &  \textbf{25.26} &      63.03 \\
%          58 &  256 &   4 &      0.00 &  25.57 &      64.89 \\
%          64 &  256 &   5 &      0.40 &  25.57 &      66.03 \\
%          58 &  256 &   4 &      0.00 &  25.57 &      67.11 \\
%          60 &  256 &   4 &      0.13 &  25.45 &      67.18 \\
%          64 &  256 &   3 &      0.00 &  26.07 &      67.40 \\
%          77 &  256 &   3 &      0.00 &  25.56 &      \textbf{68.00}\ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Various hyperparameter settings for compression near 25.5x}
%     \label{tab:cr_effect_25}
% \end{table}
%\vspace{-0.5cm}

% \begin{figure}
% \centering
% \begin{small}
% \includegraphics[width=7.5cm]{fig/per_layer_plots.pdf}
% \end{small}
% \caption{Per layer results for Resnet18}
% \label{fig:per_layer_plots}
% \end{figure}


% \subsubsection{Tiling}
% In this experiment we investigate how different methods of reshaping a convolutional weight tensor into a matrix of shape $n\times d$ affects results.
% We specifically focus on 'flattening' the weight tensor along channel dimensions, instead of filter dimensions.

% TODO: add results, still running.

% \begin{table}
% \centering
%     \begin{tabular}{c|c}
%          &  \\
%          \hline \\
%          &
%          & 
%     \end{tabular}
%     \caption{}\label{tab:lr_ablation}
% \end{table}







==> Vector quantization_/introduction.tex <==
\section{Introduction}
Deep neural networks have achieved state-of-the-art results in a wide variety of tasks.
However, deployment remains challenging due to their large compute and memory requirements.
Neural networks deployed on edge devices such as mobile or IoT devices are subject to stringent compute and memory constraints, while networks deployed in the cloud do not suffer such constraints but might suffer excessive latency or power consumption.

% A significant contributor to inference time power consumption and latency is weight data transfer.
% During weight data transfer, cores may idle as weights are being transferred from off-chip to on-chip memory.



% For this reason a wide variety of approaches to reduce compute requirements have been have been introduced in literature.


% Networks deployed in the cloud do not suffer such restrictions, but still benefit from resource usage reductions, through reduced power consumption and reduced latency.


To reduce neural network memory and compute footprint, several approaches have been introduced in literature. 
Methods related to our approach, as well as their benefits and downsides, are briefly introduced in this section and described in more detail in the related works section.
\emph{Tensor factorization} approaches \citep{denil2013predicting} replace a layer in a neural network with two layers, whose weights are low-rank factors of the original layer's weight tensor. 
This reduces the number of parameters and multiply-add operations (MACs), but since the factorizations are by design restricted to those that can be realized as individual layers, potential for compression is limited.
By \emph{pruning} a neural network \citep{louizos2017learning,he2017channel}, individual weights are removed. 
% While this in theory reduces model size, in practice networks with random sparsity do not automatically lead to space savings due to hardware restrictions.
Pruning has shown to yield moderate compression-accuracy trade-offs.
Due to the overhead required to keep track of which elements are pruned, real yield of (unstructured) pruning is lower than the pruning ratio.
An exception to this is \emph{structured pruning}, in which entire neurons are removed from a network, and weight tensors can be adjusted accordingly. 
However, achieving good compression ratios at reasonable accuracy using structured pruning has proven difficult.
\emph{Scalar quantization} \citep{Jacob2018quantization,Nagel2021AWP} approximates neural network weights with fixed-point values, i.e., integer values scaled by a fixed floating point scalar. 
Scalar quantization has shown to yield high accuracy at reasonable compression ratios, e.g., 8 bit quantization yields a 4x compression ratio and virtually no accuracy degradation on many networks. However, scalar quantization does not yield competitive compression vs accuracy trade-offs at high compression ratios.
\emph{Vector quantization} \citep{stock2019and,martinez2021permute} approximates small subsets of weights, e.g., individual $3 \times 3$ filters in convolutional weight tensors, by a small set of codes. 
This way, the storage can be reduced by storing the codebook and one code index for each original vector, instead of the individual weights. 
%For example, if there are $K$ codes, storage requirement of code indices is $\log_2(K)$ bits per $3\times 3$ filter. 
While vector quantization can achieve high compression with moderate accuracy loss, these methods usually struggle to reach the accuracy of uncompressed models in low compression regimes. 

% A number of relevant methods are briefly introduced here, and will be discussed more in-depth in the related works section.

% Move details to related work, focus on why these methods need improvement (in terms of accuracy vs 

% \textcolor{blue}{Andrey: I moved part of the text which introduces different methods to the related work. Maybe we should have here one big paragraph which discusses only the limitations of the described approaches? Another approachs would be to move the limitations to the related work as well, but then we need to add some kind of motivating parapgraph to the introduction.}
% \textcolor{blue}{Limitations of SVD}: Traditionally, tensor factorization is implemented as two consecutive neural network layers, where each tensor factor is used as the weight of one of the new layers.
% This implementation choice severely restricts the potential factorizations that can be applied and thus reduces applicability of this approach.

% \textcolor{blue}{Limitations of unstructures pruning}:In case sparsity is applied structurally, e.g. by removing entire neurons or activation maps, a reduced memory footprint is easily achieved. 
% However, in case sparsity is not applied in an unstructured fashion, different data structures, e.g. compressed sparse row/column or bit-flags for zero weights, must be employed to yield a reduced memory footprint.

% \textcolor{blue}{Limitations of scalar quantization}:By using per-channel weight quantization, i.e. using a separate quantization scale for each output neuron or output map, dramatically higher scores can be achieved with a negligible increase in memory footprint.
% However, while quantization works well at relatively low compression ratios, results degrade quickly for higher compression ratios. 

% \textcolor{blue}{Limitations of VQ}:
% Vector quantization approximates small subsets of weights, e.g. individual $3 \times 3$ filters in convolutional weight tensors, by a small set of codes. 
% This way, storage can be reduced by storing the codebook and one code index for each original vector, instead of the individual weights. For example, if there are $K$ codes, storage requirement of code indices is $\log_2(K)$ bits per $3\times 3$ filter. 
% While vector quantization can achieve moderate accuracy loss in high compression regimes, these methods usually struggle to reach the accuracy of uncompressed models in low compression regimes.
% \begin{figure}[t]
% \centering
% \begin{small}
% \begin{tabular}{c}
% \includegraphics[width=8.0cm]{fig/sparse_pca_figure.pdf}
% \label{fig:sparse_pca}
% \end{tabular}
% \end{small}
% \caption{An illustration on Qantized sparse PCA method. The weight tensor is reshaped into a matrix and is factorized intro a codebook and a latent. Both factors are quantized while the latent matrix is sparse.}
% \end{figure}

\begin{figure*}[t]
    \centering
        \begin{small}
            \begin{tabular}{c}
            \includegraphics[width=\linewidth]{fig/pg2-fig.pdf}
            \label{fig:sparse_pca}
            \end{tabular}
        \end{small}
    \caption{An illustration of application of Quantized Sparse PCA to a convolutional weight tensor. The weight tensor is reshaped into a matrix of shape $d\times n$ and factorized into a codebook $\mathbf{C}\in\mathbb{R}^{d\times k}$ and a latent $\mathbf{Z}\in\mathbb{R}^{k\times n}$. Both factors are quantized while only $\mathbf{Z}$ is sparse. During inference the arrows are followed backwards: the reshaped and tiled matrix is computed from the product of the factors $\mathbf{C}$ and $\mathbf{Z}$. The result is reshaped into the original weight tensor.}
\end{figure*}


% \arash{It seems that the quantization is almost not touched in this paragraph?}
In this paper, we provide a novel view on tensor factorization. 
Instead of restricting factorization to those that can be realized as two separate neural network layers, we show that much higher compression ratios can be achieved by shifting the order of operations. 
In our method, we find a factorization $\rmC, \rmZ$ for an original weight tensor $\rmW$, such that the matrix product $\rmC\rmZ$ closely approximates the original weight tensor. The compression is then pushed further by obtaining quantized factors and additionally sparse $\rmZ$.
During inference, the product $\rmC\rmZ$ is computed first, and its result is reshaped back into the original weight tensor's shape, and used for the following computations.
This approach allows the use of an arbitrary factorization of the original weight tensor.

% While this approach increases the number of operations required to run a neural network, total latency is likely to be reduced since we can drastically reduce 
% the amount of weight data transfer and instead utilize cores that would normally idle during weight transfer to generate a layer's weight from (significantly smaller) tensor factors.

We show that this approach outperforms or is on par with vector quantization in high compression regimes, yet extends to scalar quantization levels of compression-accuracy trade-offs for lower compression ratios. 


Our contributions in this paper are as follows:
\begin{itemize}
    \item We show that the problem of tensor factorization and vector quantization can be formulated in a unified way as quantized sparse \ac{PCA} problem.
    \item We propose an iterative projected gradient descent method to solve the quantized sparse \ac{PCA} problem. 
    \item Our experimental results demonstrate the benefits of this approach. By simultaneously solving tensor factorization and vector quantization problem, we can achieve better accuracy than vector quantization in low compression regimes, and higher compression ratios than scalar quantization approaches at moderate loss in accuracy. 
\end{itemize}

% Our contributions in this paper are as follows:
% \begin{itemize}
%     \item A unified view of tensor factorization and vector quantization
%     \item A novel sparse quantized \ac{PCA} approach of weight factorization taking this view into account, furthermore drawing on the extensive literature on sparse \ac{PCA} and neural network quantization.
%     \item Experimental validation of our method showing that we can achieve better accuracy in low compression results than vector quantization, and higher compression ratios at moderate loss in accuracy than scalar quantization approaches on a number of models.
% \end{itemize}

==> Vector quantization_/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand*{\inner}[2]{\left\langle#1,#2\right\rangle}
% \newcommand*{\norm}[1]{\left\|#1\right\|}

% Theorems and Styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{lemma}[theorem]{Lemma}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{xca}[theorem]{Exercise}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

==> Vector quantization_/method.tex <==
%\vspace{-0.4cm}
\section{Method}
\label{sec:methodoutline}
%\vspace{-0.3cm}
In this section, we describe the main algorithm, which can be considered as sparse quantized \acf{PCA}.
% This section contains a general description of each step, implementation details of each step are provided in section \ref{sec:experiments}.
\vspace{-0.2cm}
\subsection{Quantized Sparse \ac{PCA}}\label{sec:quantizedpca}
%\vspace{-0.2cm}
Consider a weight tensor of a convolutional layer $\rmW \in \mathbb{R}^{f_{out} \times f_{in} \times h \times w} $, where $f_{in}$, $f_{out}$ are the number of input and output feature maps, and $h$, $w$ are the spatial dimensions of the filter. We reshape it into a matrix $\widetilde{\rmW}\in\mathbb{R}^{d \times n}$, where $d$ is the tile size and $n$ is the number of tiles. For the reshape, we consider the dimensions in the order $f_{out}, f_{in}, h, w$ in our experiments. The goal is to factorize $\widetilde{\mathbf{W}}$ into the product of two matrices as follows:
% \textcolor{red}{maybe reshape it to $d\times n$ from the beginning to avoid all the transpose.}
\begin{equation}
\widetilde{\mathbf{W}} = \mathbf{C} \mathbf{Z},
\end{equation}
where $\mathbf{C} \in \R^{d \times k}$ is the codebook, and $\mathbf{Z} \in \R^{k \times n}$ is the set of linear coefficients, or a latent variable ($k < d < n$). Following the standard PCA method, we factorize the zero mean version of $\widetilde{\mathbf{W}}$. With this decomposition, every column of $\widetilde{\mathbf{W}}$, denoted by ${\widetilde{\mathbf{W}}}_{:, i}$, is a linear combination of $k$ codebook vectors (columns of $\mathbf{C})$:
\begin{equation}
\widetilde{\mathbf{W}}_{:, i} = \sum_{j=1}^{k}\emZ_{ji}\mathbf{C_{:, j}}, 
\end{equation}
where ${\mathbf{C}}_{:,j}$ is the $j$-th column of $\mathbf{C}$. This decomposition problem is an instance of sparse \ac{PCA} methods~(\cite{zou2006sparse}). For network compression, we are additionally interested in quantized matrices $\mathbf{C}$ and $\mathbf{Z}$.
The quantization operation for an arbitrary $\mathbf{C}$ and $\mathbf{Z}$ is defined as follows:
\begin{align}
\label{eq:sparse_quant_pca}
\mathbf{C}_q & = Q_{c}(\mathbf{C};\vs_{c}, b_{c}),\\
\mathbf{Z}_q & = Q_{z}(\mathbf{Z};\vs_{z}, b_{z}),
\end{align}
%
% We efficiently, we quantize them, so that 
%
% \begin{equation}
% \label{eq:sparse_quant_pca}
% \widetilde{\rmW}}} = Q_{c}(\rmC;\vs_{c}, b_{c}) Q_{z}(\rmZ;\vs_{z}, {b}_{z}), 
% \end{equation}
where $b_c$,$b_z$ are the quantization bit-widths, and $\mathbf{s}_{c}$ and $\mathbf{s}_{z}$ are the quantization scale vectors for $\mathbf{C}$ and $\mathbf{Z}$, respectively. We consider per-channel quantization, i.e., the quantization scale values are shared for each column of $\mathbf{C}$ and each row or column of $\mathbf{Z}$ (see section \ref{sec:compression_rate} for details on which is used when):
%
\begin{equation}
\emC_{q,ij}=\mbox{clamp} \left( \left\lfloor \frac{\emC_{ij}}{s_{i}} \right\rceil , 0, 2^{b_c} - 1\right)s_{i},
\end{equation}
%
\begin{equation}
\emZ_{q,ij}=\mbox{clamp} \left( \left\lfloor \frac{\emZ_{ij}}{s_{j}} \right\rceil , 0, 2^{b_z} - 1\right)s_{j},
\end{equation}
where $\lfloor \cdot \rceil $ is rounding to nearest integer, and {$\mbox{clamp}(\cdot)$} is defined as:
\begin{equation}
\mbox{clamp}(x,a,b)= \begin{cases} 
      a & x < a \\
      x & a \leq x \leq b \\
      b & x > b 
      \end{cases}.
\end{equation}

We refer to the problem of finding quantized factors $\mathbf{C}$ and $\rmZ$ with sparse $\rmZ$ as quantized sparse \ac{PCA} problem. Once we obtain the factors $\rmC$ and $\rmZ$, we get the matrix $\widetilde{\mW}=(\rmC\rmZ)$, which can be reshaped back to a convolutional layer. The reshaped convolutional layer for factors $\rmC,\rmZ$ is denoted by $[\rmC\rmZ]$. It is well known in network compression literature that it is better to find the best factorization on the data manifold~(\cite{zhang2015accelerating,he2017channel,stock2019and}). Therefore, we solve the following optimization problem:
% \textcolor{blue}{How about $C_q$ instead of $C$ and then $C$ instead of $C_1$? Is there a clash between sparsity and the quantization scalar or is it fine like this?}:
\begin{align}
\rmC^*,\rmZ^* & = \underset{\rmC_q,\rmZ_q}{\text{argmin}} \,\,\E_{(\mX,\mY)\sim\gD}\left(\norm{\rmY-[\rmC_q\rmZ_q]*\mX}^2_F\right) \label{eq:quantize_sparse_PCA_pblm}\\
\text{s.t.}& \quad \rmC_q = Q_{c}(\rmC;\vs_{c}, b_{C}) \nonumber\\
& \quad \rmZ_q = Q_{z}(\rmZ;{\vs}_{z}, b_{Z})\nonumber\\
&\quad  \norm{\rmZ_q}_0\leq S, \rmZ\in\R^{k\times n}, \rmC\in\R^{d\times k}\nonumber,
\end{align}
where the parameter $S$ controls the sparsity ratio of $\rmZ$, $\mathbf{X}$ and $\rmY$ are the stored input output of the target layer in the original model, $\gD$ is the data distribution, and $*$ is the convolution operation. $L_0$ norm is used for the constraint on the number of nonzero elements in the matrix $\mathbf{Z_q}$. We approximate the expected value of above optimization problem using a subset of the training data:
%\[
%\norm{\mathbf{Y}_i-[\mathbf{C}_q\mathbf{Z_q}]*%\mathbf{X_i}}^2_F,
%\E_{(\mathbf{X},\mathbf{Y})\sim\gD}\left(\norm{\mathbf{Y}-[\mathbf{C_q}\mathbf{Z_q}]*\mathbf{X}}^2_F\right) \\ \approx \newline
%\frac{1}{m}\sum_{i=1}^m %\norm{\mathbf{Y}_i-[\mathbf{C}_q\mathbf{Z_q}]*\mathbf{X_i}}^2_F,
%\]

\begin{equation}
  \begin{aligned}[b]
      & \E_{(\mathbf{X},\mathbf{Y})\sim\gD}\left(\norm{\mathbf{Y}-[\mathbf{C_q}\mathbf{Z_q}]*\mathbf{X}}^2_F\right) \approx\\
      & \frac{1}{m}\sum_{i=1}^m \norm{\mathbf{Y}_i-[\mathbf{C}_q\mathbf{Z_q}]*\mathbf{X_i}}^2_F,
  \end{aligned}
\end{equation}

where $m$ is the number of samples used for optimization. Following the compression method introduced in~\cite{zhang2015accelerating}, we use output of the previous compressed layer as $\mX$ instead of the stored input to the layer in the original model. This approach aims at compensating for the error accumulation in deep networks.


%\begin{align}
%\mathbf{C}^*,\mathbf{Z}^* & = \underset{\mathbf{C}_q,\mathbf{Z}_q}{\text{argmin}} \norm{\mathbf{Y}-[\mathbf{C_q}\mathbf{Z}_q]*\mathbf{x}}^2_F \label{eq:quantize_sparse_PCA_pblm}\\
%\text{s.t.}& \quad \mathbf{C}_q = Q_{c}(\mathbf{C};\mathbf{s}_{c}, b_{C}) %\nonumber\\
%& \quad \mathbf{Z}_q = Q_{z}(\mathbf{Z};{\mathbf{s}}_{z}, b_{Z})\nonumber\\
%&\quad  \norm{\mathbf{Z}_q}_0\leq S, \mathbf{Z}\in\R^{k\times n}, \mathbf{C}\in\R^{d\times k}\nonumber,
%\end{align}
%\begin{equation}
%\underset{\mathbf{C,Z},\norm{\mathbf{Z}}_0\leq S}{\text{argmin}} \norm{\mathbf{Y}- Q_{c}(\mathbf{C};\mathbf{s}_{c}, b_{C})  Q_{z}(\mathbf{Z};{\mathbf{s}_{z}, b_{Z})[\mathbf{x}]}}^2_F 
%\end{equation}

\subsubsection{Projected Gradient Descent Optimization Algorithm}\label{sec:qs_pca_solver}

The above optimization problem can be solved using an iterative projected gradient descent method. The projection step is a hard thresholding operation which project onto the space of sparse matrices. The optimization algorithm is given below.


%\begin{algorithm}[tb]
%   \caption{Bubble Sort}
%   \label{alg:example}
%\begin{algorithmic}
%   \STATE {\bfseries Input:} data $x_i$, size $m$
%   \REPEAT
%   \STATE Initialize $noChange = true$.
%   \FOR{$i=1$ {\bfseries to} $m-1$}
%   \IF{$x_i > x_{i+1}$}
%   \STATE Swap $x_i$ and $x_{i+1}$
%   \STATE $noChange = false$
%   \ENDIF
%   \ENDFOR
%   \UNTIL{$noChange$ is $true$}
%\end{algorithmic}
%\end{algorithm}

\begin{algorithm}
\caption{Projected Gradient Descent Optimization}\label{alg:projected_gd}
\begin{algorithmic}[1]
%%\item 1
\REQUIRE $\widetilde{\mathbf{W}}$
% \Ensure $y = x^n$
\STATE SVD of $ \widetilde{\mathbf{W}} = \mathbf{U}\mathbf{\Sigma}\mathbf{V}^\top,$
\STATE $\mathbf{C} \gets \mathbf{U}_k$
\STATE $\mathbf{Z} \gets \mathbf{U}_k^\top\widetilde{\mathbf{W}}$
\WHILE{Stopping criteria not met}
    \STATE \textbf{Gradient descent step:} 
   $\mathbf{C}, \mathbf{Z} \gets $ gradient descent update on equation (\ref{eq:data_sparse_pca_objective}).
%\STATE \textbf{Quantization step:} $\mathbf{C}, \mathbf{Z} \gets Q_{c}(\mathbf{C};\mathbf{s}_{c}, b_{C}), Q_{z}(\mathbf{Z};{\mathbf{s}}_{z}, b_{Z}) $.
    \STATE $\mathbf{M} \gets$ binary mask for largest $S$ values of  $Q_{z}(\mathbf{Z};{\mathbf{s}}_{z}, b_{Z})$.
    \STATE \textbf{Hard thresholding step:} 
    $\mathbf{Z} \gets  \mathbf{Z}\odot\mathbf{M}$.
\ENDWHILE
    \STATE \textbf{return:} $ Q_{c}(\mathbf{C};\mathbf{s}_{c}, b_{C}), Q_{z}(\mathbf{Z};{\mathbf{s}}_{z}, b_{Z}) $.

\end{algorithmic}
\end{algorithm}

\begin{enumerate}
    %% Initialization
    \item \textbf{Initialization.} 
    The codebook $\rmC$ is initialized with first $k$ left singular vectors of $\widetilde{\rmW}$. Given the SVD decomposition of $\widetilde{\rmW}$ as follows:
    \begin{equation}
    \widetilde{\rmW} = \mathbf{U}\mathbf{\Sigma}\mathbf{V}^\top,
    \end{equation}
    we choose $\rmC^{(0)} = \mathbf{U}_k$, where $\rmU_k$ denotes the top $k$ left singular vectors of $\widetilde{\rmW}$. The latent matrix $\rmZ$ is initialized as the projection of $\widetilde{\rmW}$ onto the set of first $k$ singular vectors, $\rmZ^{(0)} =\rmU_k^\top \widetilde{\rmW}$.
    % The codebook $\rmC$ is initialized with first $k$ right singular vectors of $\widetilde{\mW}^T$. Given the SVD decomposition of $\widetilde{\mW}^T$ as follows:
    % \begin{equation}
    % \widetilde{\mW}^T = \mathbf{U}\mathbf{\Sigma}\mathbf{V^T},
    % \end{equation}
    % we choose $\rmC^{(0)} = \mathbf{V}^T$. The latent matrix $\rmZ$ is initialized as the projection of $\rmW$ onto the set of first $k$ singular vectors, $\rmZ^{(0)} = \widetilde{\rmW}\mV$.
    %% Gradient descent
    \item \textbf{Gradient Descent.} At iteration $t$, the matrices $\rmC^{(t-1)},\rmZ^{(t-1)}$ are updated by gradient descent on the following objective w.r.t. $\rmC$ and $\rmZ$:
    \begin{equation}
    \frac{1}{m}\sum_{i=1}^m \norm{\rmY_i- [Q_{c}(\rmC;\vs_{c}, b_{C})  Q_{z}(\rmZ;{\vs}_{z}, b_{Z})]*\rmX_i]}^2_F,
    \label{eq:data_sparse_pca_objective}
    \end{equation}
    We use the \ac{STE} (\cite{bengio_estimating_2013}) to compute the gradients of the quantization operation, i.e. we use the following gradient estimate for the rounding operation: 
    \begin{equation*}
    \frac{\partial \lceil p\rfloor}{\partial p}=1.
    \end{equation*}
    
    The outcome of this step is denoted by $\rmC^{(t)}_{\text{gd}},\rmZ^{(t)}_{\text{gd}}$.
    % %% Quantization
    % \item \textbf{Quantization.} The matrices $\rmC^{(t)}_{\text{gd}},\rmZ^{(t)}_{\text{gd}}$ are projected onto the space of quantized matrices:
    % \[
    % \rmC_q^{(t)}= Q_{c}(\rmC^{(t)}_{\text{gd}};\vs_{c}, b_{C}), \quad
    % \rmZ_q^{(t)}= Q_{z}(\rmZ^{(t)}_{\text{gd}};{\vs}_{z}, b_{Z})
    % \]
    \item \textbf{Hard thresholding.} 
    After the gradient descent, we project $\rmZ^{(t)}_{\text{gd}}$ onto the space of sparse matrices. The projection is done using entrywise product of $\rmZ^{(t)}_{\text{gd}}$ with a binary mask matrix $\rmM^{(t)}$, namely  $\rmZ^{(t)}_{\text{gd}}\odot \rmM^{(t)}$. 
    The mask matrix $ \mM^{(t)}$ is obtained finding the support of $S$ largest entries of $Q_{z}(\rmZ^{(t)}_{\text{gd}};{\vs}_{z}, b_{Z})$. This is the hard thresholding step. For the next iteration we set:  \[
    \rmZ^{(t)}=\rmZ^{(t)}_{\text{gd}}\odot \mM^{(t)}, \rmC^{(t)}=\rmC^{(t)}_{\text{gd}}.
    \]
    % onto the space of sparse matrices. The projection is done using hard thresholding, which is based on selecting top $S$ values of the quantized values of $\rmZ_2^{(t)}$. Denote the threholding operation by $H_S(.)$. This step is then given by  
    % \[
    % \rmZ^{(t)}=H_S(\rmZ_q^{(t)})
    % \]
    % Set $\rmC^{(t)}=\rmC_q^{(t)}$.

    % After the gradient descent and quantization steps, we project $\rmZ_q^{(t)}$ onto the space of sparse matrices. The projection is done using hard thresholding, which is based on selecting top $S$ values of the quantized values of $\rmZ_2^{(t)}$. Denote the threholding operation by $H_S(.)$. This step is then given by  
    % \[
    % \rmZ^{(t)}=H_S(\rmZ_q^{(t)})
    % \]
    % Set $\rmC^{(t)}=\rmC_q^{(t)}$.
    \item Repeat the previous three steps using $\rmZ^{(t)},\rmC^{(t)}$ until termination criteria is met (MSE error or a fixed iterations number). The final matrices are given be     $Q_{c}(\rmC^{(t)};\vs_{c}, b_{C}), Q_{z}(\rmZ^{(t)};{\vs}_{z}, b_{Z})$.
% We then sparsify $\rmZ$ by applying hard thresholding on the (unquantized) values of $\rmZ$.
% Lastly, $\rmC$ and $\rmZ$ are quantized as explained in section 2.1. We refer the reader to Appendix \ref{sec:hard_thresholding} details on hard thresholding
\end{enumerate}

%The termination criteria can be either based on MSE error on a subset of data or a simple bound on the iteration number. 

It is in general difficult to provide convergence analysis for non-convex optimization problems such as (\ref{eq:quantize_sparse_PCA_pblm}). Iterative thresholding methods are, however, widely used to solve sparse optimization problems \cite{jacques2013robust,foucart_mathematical_2013}, and in some cases, they have theoretical guarantees. In
Appendix \ref{sec:hard_thresholding}, we discuss some of the results. Note that the theory does not apply directly to our setup. Nonetheless, it provides intuition behind effectiveness of the proposed approach.

%\begin{equation}
%w_{ij} = \sum_{j=1}^{k}Q_{\alpha}(\alpha_{i,j};s_{\alpha}, b_{\alpha}) %Q_{u}(u_{i,j};s_{u}, b_{u}) + u_{i0}      
%\end{equation}
%\vspace{-0.25cm}
\begin{figure*}[ht]
\centering
\begin{small}
\begin{tabular}{l}
\hspace{-0.2cm}\includegraphics[width=0.9\textwidth]{fig/resnet18_plots_cinematic.pdf} \\
\end{tabular}
\end{small}
\caption{Results for Resnet18 trained on ImageNet.}
\label{fig:resnets_plots}
\end{figure*}
\subsubsection{Relation to other approaches}
In this section, we discuss the connection with other existing methods. 
\begin{enumerate}
    
    \item[(A)] \textbf{Vector quantization.}
        If we replace the quantizers for $\rmC$ and $\rmZ$ by identity functions, i.e. $Q_c= \mbox{id}(\cdot)$, $Q_{z}= \mbox{id}(\cdot)$, then matrix $\rmC$ is in full precision, while $\rmZ$ encodes the indices such that
        \begin{equation}
        \emZ_{ij}=\delta_{im_i},
        \end{equation}
        where $m_i$ is the centroid index corresponding to tile $i$.
        
    \item[(B)] \textbf{Additive vector quantization.}
        If $Q_c= \mbox{id}(\cdot)$, $b_{z}= 1$ (binary quantization), then
        \begin{equation}
        \widetilde{\rmW}_{:,i} = \sum_{j=1}^{k}\rho_{ji}\rmC_{:,j}, 
        \label{eq:additivevq}
        \end{equation}
        where $\rho_{ji} \in \{0,1\}$ are binary coefficients. 
        Note that in the original work by~\cite{babenko2014additive}, an additional constraint of $\sum_j \rho_{ji}=n_t$ is enforced, i.e. each $\rmW_{i,:}$ is a sum of a fixed number of terms.
    
    %If values $\rho_{ij}$ are highly sparse, this case corresponds to additive vector quantization.
    
    \item[(C)] \textbf{Principle component analysis.}
        If $Q_{c}= \mbox{id}(\cdot)$, and $Q_z= \mbox{id}(\cdot)$, then
        \begin{equation}
        \widetilde{\rmW}_{:,i} = \sum_{j=1}^{k}\emZ_{ji}\rmC_{:, j}. 
        \end{equation}\label{eq:pca}
        This case corresponds to SVD factorization of zero mean version of weight matrix $\widetilde{\rmW}$. For specific values of $n$ and $d$, the method is mathematically equivalent to the SVD decomposition methods for neural network compression~(\cite{denton2014exploiting, jaderberg2014speeding}). For example, if $n=f_{out}h$, and $d=f_{in}w$, then the method is equivalent to the spatial SVD decomposition by~\cite{jaderberg2014speeding}. In contrast to the above-mentioned approaches, we do not decompose the convolutional operation into two convolutional layers, which gives extra flexibility in the choice of PCA dimensionality $d$. 

\end{enumerate}

\subsection{Compression ratio}\label{sec:compression_rate}
%\vspace{-0.25cm}
Without sparsity, the compression ratio is computed as follows.
Let $L_o(\rmW) = f_{out}\times f_{in} \times h \times w \times 32$ denote the number of bits required to represent the original 32 bit floating point tensor $\rmW$, and $L_c(\rmW) = d\times k \times b_c + k \times n \times b_z$ the size of the quantized tensor factors $\rmC$ and $\rmZ$ of $\rmW$.
The compression ratio $C_r$ is then defined as $C_r=\frac{L_o(\rmW)}{L_c(\rmW)}$.

Note that, since $k < d < n$, the latent matrix $\rmZ$ contributes more to the resulting model size than the codebook matrix $\rmC$. 
For example, let us assume $f_{out} = f_{in} = 256$, $h = w = 3$, $d=256$, and $k=128$. 
In this scenario, the original weight tensor $\rmW$ has $256\times256\times3\times3=589,824$ elements, the codebook matrix $\rmC$ has $256\times128=32,768$ elements and the latent matrix $\rmZ$ has $128 \times 2,034=260,356$ elements, almost 8 times as many as $\rmC$.
For this reason, efforts to compress $\rmZ$, e.g., by using a lower bitwidth $b_c$ or pruning elements, will likely yield a better accuracy vs compression trade-off than focusing similar efforts on $\rmC$.

Additional compression is achieved by encoding the  sparse matrix $\rmZ$ as follows.
We assume the sparsity mask $\rmM$ is stored as a binary matrix.
Then, we only store the nonzero values in $\rmZ$.
At runtime, $\rmZ$ can be decoded by only reading values in $\rmZ$ for which the corresponding binary mask value is equal to $1$.
The total number of bits required to store $\rmM$ and the nonzero values in $\rmZ$ is $k\times n + (1-r) \times k\times n \times b_z$, where $r=1-S/kn$ is the sparsity ratio of $\rmZ$ with $\norm{\rmZ}_0=S$.
Note that this method only reduces memory footprint if $r > 1/b_z$.

The size of the compressed tensor must be adjusted for quantization parameters introduced by per-channel quantization. 
We assume that each quantization scale parameter is encoded using FP16. 
% We find that using a quantizer for each column of $\rmZ$ yields better accuracy, but increases model size disproportionately at high compression ratios.
% Therefore, we use separate quantizers for each column of $\rmZ$ in low compression regimes, and separate quantizers for each row of $\rmZ$ in high compression regimes.
To account for this we add a quantization adjustment term $L_q(\rmW)$ to $L_c(\rmW)$, where $L_q=2k\times 16$ is used for per-row quantization of $\rmZ$.
%and $L_q=(k+n)\times 16$ is used for per-column quantization of $\rmZ$.

Finally, taking into account the adjustments for sparsity and quantization parameters, the size of a compressed tensor is computed as $L_c(\rmW)=d\times k \times b_c + k\times n + (1-r)\times k \times n \times b_z  + L_q(\rmW)$.

\subsection{Computational overhead}\label{sec:computational_overhead}
The complexity of the forward pass for a convolutional layer is $f_{in}f_{out}hwp$. The overhead for the filter reconstruction is the product of two matrices using $f_{in} f_{out}hwk$ multiply-add operations (MACs). So the relative overhead in the number of operations is $k/p$. Practically, for Resnet18, a value of $k$ equals for example 128, while the spatial size of the feature map for an ImageNet goes down from $56\times 56$ to $7\times7$ in the later layers. So, the relative overhead for a single forward pass is varying between $4\%$ and $261\%$ extra operations for different layers. While the total relative overhead for the full model is $85\%$ extra MACs. However, with an increasing batch size or when doing multiple inferences this becomes neglectable.
The comparison above is based on MACs, however in our approach, most computations contain low bit tensors. If we do the same comparison in bit operations (BOPs) the overhead is significantly reduced.
% \subsubsection{Equality of Additive VQ and quantized \ac{PCA}}
% \arash{Let's talk about this section. I have some questions. The notation is diverging from previous sections.}
% We can binarize of shape $\rmZ^{int} \in \mathbb{R}^{k\times n}$, where $Z^{int}_{ij}=\text{clamp}\left( \lfloor\frac{Z_{ij}}{s_j}\rceil, 0, 2^b - 1
% \right)$ by replacing it with a tensor $\widehat{\rmZ}\in \{0, 1\}^{(b_z\cdot k) \times n}$ where element $\widehat{Z}_{ij}$ is the $i \mod b_z$th bit of $Z_{\lfloor i / b_z \rfloor}$.
% We can then rewrite equation \ref{eq:additivevq} as follows:

% \begin{equation}
%     \mathbf{w_i} = s_i \sum_j^{(b_z\times k)} \widehat{Z}_{ji}2^{j\mod b_z} \rmC_{\lfloor j / b_z \rfloor}
% \end{equation}\label{eq:binaryvq}


% \subsection{Sparse quantized \ac{PCA}.} The sparsity is introduced latent variable $\rmZ$ to eq.~\ref{eq:sparse_quant_pca} by 
% \begin{equation}
% \widetilde{\rmW}}} = Q_{c}(\rmC;\vs_{c}, \mathbf{b}_{c})\left[ \rmM \odot  Q_{z}(\rmZ;\vs_{z}, {b}_{z}) \right], 
% \end{equation}
% where $m_{ij} \in \{0,1\}$ a binary sparsity mask. The sparsity mask is applied on the quantized values in order not to enforce pruning of low magnitude non-zero values. 
% We only apply sparsification to $\rmZ$ for the reasons outlined in section \ref{sec:compression_rate}.

% \subsubsection{Initialization}.

% The codebook is initialized with first $k$ principal components of $W$, which is obtained using SVD decomposition as follows.
% \begin{equation}
% \rmW = \mathbf{U}\mathbf{\Sigma}\mathbf{V^T},    
% \end{equation}

% \begin{equation}
% \rmC = \mathbf{V_k}^T,    
% \end{equation}

% The latent matrix $\rmZ$ is initialized as the projection of $\rmW$ onto the set of first $k$ principal components:

% \begin{equation}
% \rmZ = \mathbf{WV_k}.
% \end{equation}

% We then sparsify $\rmZ$ by applying hard thresholding on the (unquantized) values of $\rmZ$.
% Lastly, $\rmC$ and $\rmZ$ are quantized as explained in section 2.1. We refer the reader to Appendix \ref{sec:hard_thresholding} details on hard thresholding

% \subsubsection{Additional compression due to sparsity}
% Additional sparsity is achieved by encoding our sparse matrix $\rmZ$ as follows.
% We assume the sparsity mask $\rmM$ is stored as a binary matrix.
% Then, we only store the nonzero values in $\rmZ$.
% At runtime, $\rmZ$ can be decoded by only reading values in $\rmZ$ for which the corresponding binary mask value is equal to $1$.
% The total number of bits required to store the nonzero values in $\rmZ$ and $\rmM$ is $k\times n + (1-r) \times k\times n \times b_z$. where $r$ is the sparsity ratio of $\rmZ$.
% Note that this method only reduces memory footprint if $r > 1/b_z$.

% \subsection{Per layer data-aware optimization}
% As next step, we obtain extra initialization step by applying data-aware optimization on the pre-activation output of the original layer.

% We solve the following optimization problem:
% \begin{equation}
% \underset{\mathbf{C,Z},\norm{\rmZ}_0\leq S}{\text{argmin}} \norm{\rmY- Q_{c}(\rmC;\vs_{c}, b_{C})  Q_{z}(\rmZ;{\vs}_{z}, b_{Z})[\mathbf{x}]}^2_F 
% \end{equation}
% where the parameter $S$ controls the sparsity ratio of $\rmZ$, $\mathbf{x}$ is a stored input of the target layer, and $\rmY$ is a stored output of this layer in the original model. 

% This optimization problem is solved using an iterative projected gradient descent method. Starting from the initialization point, we perform a gradient descent step on $\rmC,\rmZ$ by computing the gradient of the objective function w.r.t. $\rmC$ and $\rmZ$. We use the \ac{STE} as described in \cite{bengio_estimating_2013} to compute the gradients of the quantization operation. 
% After the gradient descent step, we project $\rmZ$ onto the space of sparse matrices. The projection is done using hard thresholding, which is based on selecting top $S$ values of the quantized values of $\rmZ$.  

% During optimization we iterate between the following two steps:

% Step 1: Compute the gradient of the objective function w.r.t. $\rmC$ and $\rmZ$, and perform a gradient descent step on Z and C reduce 

% Step 2: Apply hard thresholding on $Z$, on the unquantized values of $\rmZ$.  

% Note that we use the straight through estimator (STE) as described in REF to compute the gradients of the quantization operation w.r.t. $\rmC$ and $\rmZ$.


% \subsection{Our method}\label{sec:methodoutline}
% Our method combines the steps outlined in sections 2.1-2.3 as follows:

% \begin{enumerate}
%     \item We find the initial factorization using the quantized sparse \ac{PCA} approach described in section 2.2.
%     \item We then sparsify this method using hard thresholding.
%     \item We perform an initial optimization of $\rmZ$ as described in section 2.3
%     \item Lastly, we perform end-to-end fine-tuning.
% \end{enumerate}


==> Vector quantization_/related_work.tex <==
\vspace{-0.5cm}
\section{Related work}

\textbf{SVD-based methods and tensor decompositions}
SVD decomposition was first used to demonstrate redundacy in weight parameters in neural networks in~\cite{denil2013predicting}. Later several methods for reducing the inference time based on SVD decomposition were suggested ~\citep{denton2014exploiting, jaderberg2014speeding}. A similar technique was proposed for gradients compression in data-parallel distributed optimization by~\cite{vogels2019powersgd}. The main difference between these methods is the way 4D weights of a convolutional layer is transformed into a matrix which leads to different shapes of the convolutional layers in the resulting decomposition. 
Following a similar direction, several works focus on higher-order tensor decomposition methods which lead to introducing of three or four convolutional layers ~\citep{lebedev2014speeding, kim2015compression, su2018tensorized}.

\paragraph{Weight pruning}
A straightforward approach to reducing neural network model size is removing a percentage of weights.  A spectrum of weight pruning approaches of different granularity has been introduced in the literature. Structured pruning approaches such as~\cite{he2017channel} kill entire channels of the weights, while unstructured pruning approaches ~\citep{louizos2017learning, zhu2017prune, neklyudov2017structured, dai2018compressing} focus on individual values. A recent survey on unstructured pruning is provided in~\cite{gale2019state}.

% TODO: possibly talk about gradual pruning

\paragraph{Scalar quantization and mixed precision training}
By quantizing neural network weights to lower bitwidths, model footprint can be reduced as well, as each individual weight requires fewer bits to be stored.
For example, quantizing 32 bit floating points weight to 8 bit fixed point weights yields a 4x compression ratio. Most quantization approaches use the straight-through estimator (STE) for training quantized models~(\cite{bengio_estimating_2013, krishnamoorthi2018quantizing}). One way to further improve the accuracy of quantized models is learning the quantization scale and offset jointly with the network parameters~(\cite{esser2019learned, bhalgat2020lsq+}).
A recent survey on practical quantization approaches can be found in \cite{Nagel2021AWP}.

In order to improve the accuracy of quantized models, several methods suggest using mixed precision quantization. The work by~\cite{uhlich2019differentiable} introduced an approach on learning integer bit-width for each layer using STE. Using non-uniform bit-width allows the quantization method to use lower bit-width for more compressible layers of the network. Several works~\citep{van2020bayesian, dong2019hawq, wang2019haq} improve upon the approach by~\cite{uhlich2019differentiable} by using different methods for optimization over the bit-widths. 

\textbf{Vector quantization.}
Several works use vector quantization approach for compression of weights of convolutional and fully connected layers~(\cite{gong2014compressing, martinez2021permute, fan2020training, stock2019and, wu2016quantized}). The convolutional weight tensors are reshaped into matrices, then K-means methods is applied directly on the rows or columns. Besides weight compression, the work by~\cite{wu2016quantized} suggests using vector quantization for reducing the inference time by reusing parts of the computation.

Recently several works suggested improvements on the basic vector quantization approach. Data-aware vector quantization which improves the clustering method by considering input activation data is demonstrated to improve the accuracy of the compressed models by \cite{stock2019and}. Another direction is introducing a permutation to the weight matrices which allows to find subsets of weights which are more compressible~\citep{martinez2021permute}. An inverse permutation is applied at the output of the corresponding layers to preserve the original output of the model.

Besides weights compression problem, various improved vector quantization methods were applied in image retrieval domain in order to accelerate scalar product computation for image descriptors~(\cite{chen2010approximate,ge2013optimized, norouzi2013cartesian}). 
In particular, additive quantization method which we will show is related to quantized sparse PCA was introduced~\cite{babenko2014additive}. 
% Additive quantization \citep{babenko2014additive} allows for more than one codebook vector per reconstruction.
Surveys on vector quantization methods are provided in~\cite{matsui2018survey, gersho2012vector}.

\textbf{Sparse \ac{PCA}.} Introduced in \cite{zou2006sparse}, sparse \ac{PCA} can be solved by a plethora of algorithms. The method proposed in this paper can be considered as an instance of thresholding algorithms \citep{ma_sparse_2013}. Although soft-thresholding methods are prevalent in the literature, we adopt an explicit projection step using hard thresholding to have direct control over the compression ration. Note that sparse \ac{PCA} can be extended to include additional structures with sparsity \citep{jenatton_structured_2010, lee_efficient_2006}.


